AeroChem: Closed-loop Physics-Informed State Space Modeling for Long-term Chemically-Reactive Air Quality Forecasting--Extended Version

Accurate long-term air quality forecasting is challenging due to long-range transport, meteorological variability, and nonlinear chemical reactions underlying secondary pollutant formation. Purely data-driven models often suffer from long-horizon drift and lack physical consistency, while existing physics-informed approaches commonly follow open-loop designs that fuse neural and physical components only at the output level. We propose AeroChem, a closed-loop physics-informed state space framework for chemically reactive air quality forecasting. AeroChem adopts a two-branch co-correction design: a UDE-based process branch provides a structured but imperfect physical prior, while a Mamba-based virtual measurement branch captures long-range temporal context and produces probabilistic virtual observations. Neural Kalman Fusion couples the two branches by correcting the latent physical state at each forecasting step and feeding the posterior state back into the simulator, reducing long-horizon drift. We further introduce HanoiAir, a real-world dataset integrating pollutant concentrations, meteorology, and emission inventories. Experiments on HanoiAir and a public benchmark show that AeroChem improves long-horizon stability and sudden-change forecasting.

==> data/sensitivity_d_model.tex <==
# x     MAE     RMSE
64      25.30   40.06
96      24.08   39.34
128     24.50   39.66

==> data/sensitivity_dt.tex <==
# x     MAE     RMSE
0.25    33.22   49.14
0.5     27.88   45.35
0.75    25.01   41.08
1.0     24.08   39.34
1.25    27.40   43.92
1.5     37.52   57.84
2.0     54.87   81.46

==> data/sensitivity_phy_weight.tex <==
# x       MAE     RMSE
0.0       25.65   41.48
0.005     25.24   40.86
0.01      24.97   40.47
0.02      24.63   40.00
0.05      24.20   39.48
0.1       24.08   39.34
0.2       24.22   39.50
0.5       24.74   40.07
1.0       25.25   40.63

==> sections/abstract.tex <==

% \begin{abstract}
%     Accurate air quality forecasting is critical for public health, yet it faces two significant challenges: capturing long-range temporal dependencies and modeling the complex chemical formation of secondary pollutants. Existing methods are often limited, as purely data-driven models may produce physically implausible results, while current physics-informed models typically overlook non-linear chemical reactions and possess short temporal memory. To address these limitations, we propose \framework, a novel dual-branch, physics-informed deep learning framework. \framework uniquely integrates two specialized dynamics branches. The data-driven branch employs a Mamba-based State Space Model (SSM) to efficiently capture long-range seasonal and meteorological patterns from historical data. Concurrently, the physics-informed branch learns to infer the parameters of a governing Stochastic Delay Reaction-Advection-Diffusion (SD-RAD) system, solving it as a Stochastic Differential Equation (SDE) to explicitly model chemical transformations.
%     These complementary branches are synergistically combined through a confidence-aware fusion mechanism, which utilizes the SDE's predicted variance to adaptively weigh their contributions, producing a forecast that is both accurate and probabilistically reliable. Extensive experiments on large-scale, real-world air quality datasets demonstrate that \framework significantly outperforms state-of-the-art models in prediction accuracy, particularly for challenging secondary pollutants like ozone and in long-term forecasting scenarios. Our work provides a robust and principled framework for next-generation air quality forecasting, offering a promising tool for effective environmental management and public policy. We made the source code publicly available at \underline{\url{https://github.com/kiendemo/AeroChem}}.
% \end{abstract}
\begin{abstract}
    Accurate air quality forecasting is critical for public health, yet it faces two significant challenges: capturing long-range temporal dependencies and modeling the complex chemical formation of secondary pollutants. Existing methods are often limited, as purely data-driven models may produce physically implausible results, while current physics-informed models typically overlook non-linear chemical reactions and possess short temporal memory. To address these limitations, we propose \framework, a novel closed-loop, physics-informed deep learning framework. 
    \framework integrates two specialized components within a Data Assimilation paradigm. The data-driven branch acts as a virtual sensor, employing a Mamba-based State Space Model (SSM) to extract global spatiotemporal contexts from historical data. Concurrently, the physics-informed process model utilizes a Universal Differential Equation (UDE) to explicitly disentangle transport from reaction dynamics, featuring a novel  Neural Reaction mechanism that mimics chemical kinetics. Crucially, these branches are unified via a Neural Kalman Fusion module. Unlike previous loose-coupling approaches, our framework operates as a closed-loop system, where the fused posterior state is recursively fed back into the physics engine to continuously correct the trajectory and mitigate error accumulation in long-term forecasting. Extensive experiments on large-scale, real-world air quality datasets demonstrate that \framework significantly outperforms state-of-the-art models in prediction accuracy, particularly for challenging secondary pollutants like ozone and in long-term forecasting scenarios. Our work provides a robust and principled framework for next-generation air quality forecasting, offering a promising tool for effective environmental management and public policy. We made the source code publicly available at \underline{\url{https://github.com/kiendemo/AeroChem}}.
\end{abstract}


==> sections/appendices.tex <==
\appendix
\section{Appendix}
\subsection{Algorithmic Summary of \framework}
\label{app:sec:algorithm}

We provide a step-by-step algorithmic summary of the \framework framework.
Algorithm~\ref{alg:aerochem} details the closed-loop forecasting procedure, explicitly illustrating how the measurement model, the physics-informed Universal Differential Equation (UDE), and the Neural Kalman Fusion module interact over the forecasting horizon.
The algorithm highlights the recursive feedback mechanism in which posterior latent states are assimilated and fed back into the UDE solver.

\begin{algorithm}[h]
\caption{AeroChem Forecasting}
\label{alg:aerochem}
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Sensor graph $\mathcal{G}$; historical observations $\mathbf{X}_{1:T_{\text{in}}}$; meteorology $\mathbf{M}_{1:T_{\text{out}}}$; emissions $\mathbf{E}_{1:T_{\text{out}}}$; forecast horizon $T_{\text{out}}$.}
\Output{Forecasted observations $\hat{\mathbf{X}}_{T_{\text{in}}+1:T_{\text{in}}+T_{\text{out}}}$.}

\BlankLine
\textbf{Measurement encoding:}\;
$\mathbf{H}_{\text{ctx}} \leftarrow \text{S-Mamba}(\mathbf{X}_{1:T_{\text{in}}})$\;
$(\mathbf{Z}_{\text{base}}, \mathbf{R}_{\text{base}}) \leftarrow \text{ProjHeads}(\mathbf{H}_{\text{ctx}})$\;

\BlankLine
\textbf{Initialization:}\;
Initialize posterior latent state $\mathbf{S}^+_{0}$ (e.g., from the last observed timestep via a projection/encoder)\;

\BlankLine
\For{$t \leftarrow 1$ \KwTo $T_{\text{out}}$}{
    \textbf{Adaptive virtual observation:}\\
    $\mathbf{Z}_{\text{obs},t} \leftarrow \mathbf{Z}_{\text{base}} + \alpha \tanh(\mathbf{S}^+_{t-1})$\\
    $\mathbf{R}_{\text{obs},t} \leftarrow \text{Softplus}(\mathbf{R}_{\text{base}})\left(1 + \beta \frac{t}{T_{\text{out}}}\right)$

    \BlankLine
    \textbf{UDE prediction (time update):}\\
    $\mathbf{S}^-_t \leftarrow \text{UDE-Solve}\!\left(\mathbf{S}^+_{t-1}; \mathbf{M}_t, \mathbf{E}_t, \mathcal{G}\right)$\\
    $\mathbf{P}^-_t \leftarrow \text{Softplus}(\text{Linear}(\mathbf{S}^-_t))$

    \BlankLine
    \textbf{Neural Kalman fusion (measurement update):}\\
    $\mathbf{K}_t \leftarrow \mathbf{P}^-_t / (\mathbf{P}^-_t + \mathbf{R}_{\text{obs},t})$\\
    $\boldsymbol{\epsilon}_t \leftarrow \mathbf{Z}_{\text{obs},t} - \mathbf{S}^-_t$\\
    $\boldsymbol{\epsilon}'_t \leftarrow \boldsymbol{\epsilon}_t + \text{Linear}\!\left([\mathbf{S}^-_t, \mathbf{Z}_{\text{obs},t}]\right)$\\
    $\mathbf{S}^+_t \leftarrow \mathbf{S}^-_t + \mathbf{K}_t \odot \boldsymbol{\epsilon}'_t$\\
    $\mathbf{P}^+_t = (\mathbf{1} - \mathbf{K}_t) \odot \mathbf{P}^-_t$
}

\BlankLine
\textbf{Decoding:}\;
$\hat{\mathbf{X}}_{T_{\text{in}}+1:T_{\text{in}}+T_{\text{out}}} \leftarrow \text{Decoder}(\{\mathbf{S}^+_t\}_{t=1}^{T_{\text{out}}})$\;

\Return $\hat{\mathbf{X}}_{T_{\text{in}}+1:T_{\text{in}}+T_{\text{out}}}$\;
\end{algorithm}

\subsection{HanoiAir Dataset Details}
\label{app:hanoiair}

The HanoiAir dataset provides hourly measurements from 27 monitoring stations located across various provinces in northern Vietnam, collected by the Northern Centre for Environmental Monitoring \footnote{\url{https://cem.gov.vn/}} \footnote{\url{https://vea.mae.gov.vn/}}. The data spans from January 1, 2018, to December 31, 2025 (approx. 70,128 hours).

The dataset integrates three types of data aligned temporally and spatially:
\begin{itemize}
    \item \textbf{Air Quality Observations:} Includes target pollutants PM\textsubscript{2.5} ($\mu g/m^3$), O\textsubscript{3} ($\mu g/m^3$), PM\textsubscript{10} ($\mu g/m^3$), and key precursor gases NO\textsubscript{x} ($\mu g/m^3$), SO\textsubscript{2} ($\mu g/m^3$), CO (mg/Nm³), along with NO ($\mu g/m^3$) and NO\textsubscript{2} ($\mu g/m^3$) components. The inclusion of precursor measurements (NO\textsubscript{x}, SO\textsubscript{2}, CO) is a key feature of this dataset for modeling secondary formation chemistry directly from observations.
    \item \textbf{Meteorological Variables:} Temperature (°C), Atmospheric Pressure (hPa), Solar Radiation (W/m²), Relative Humidity (\%), Wind Direction (°), Wind Speed (m/s).
    \item \textbf{Emission Data:} Includes hourly-downscaled emission rates for NO\textsubscript{x}, VOC, SO\textsubscript{2}, NH\textsubscript{4}, and primary PM\textsubscript{2.5} (tons/hour or similar unit, spatially allocated to station locations). 
\end{itemize} 
Standard pre-processing and temporal feature engineering were applied within the \texttt{BasicTS} framework~\cite{DBLP:journals/tkde/ShaoWXWYZYSJCCJC25}. The combined dataset provides the necessary inputs (observed concentrations, meteorological drivers, and emission source terms) for the physics-informed branch of \framework{} to model secondary pollutant formation.

% \subsection{Spatial Graph Construction}

% \label{app:hanoiair}


\subsection{Metric Definitions}
\label{app:metrics}

Let $\mathbf{X} \in \mathbb{R}^{T_{\text{out}} \times N}$ represent the ground truth values and $\hat{\mathbf{X}} \in \mathbb{R}^{T_{\text{out}} \times N}$ represent the predicted values for a given pollutant concentration across $N$ stations over $T_{\text{out}}$ time steps. The evaluation metrics are defined as:

\textbf{Mean Absolute Error (MAE):}
\begin{equation}
    \text{MAE}(\mathbf{X}, \hat{\mathbf{X}}) = \frac{1}{N \times T_{\text{out}}} \sum_{t=1}^{T_{\text{out}}} \sum_{n=1}^{N} |x_{t,n} - \hat{x}_{t,n}|
\end{equation}

\textbf{Root Mean Square Error (RMSE):}
\begin{equation}
    \text{RMSE}(\mathbf{X}, \hat{\mathbf{X}}) = \sqrt{\frac{1}{N \times T_{\text{out}}} \sum_{t=1}^{T_{\text{out}}} \sum_{n=1}^{N} (x_{t,n} - \hat{x}_{t,n})^2}
\end{equation}

\textbf{Symmetric Mean Absolute Percentage Error (SMAPE):}
\begin{equation}
    \text{SMAPE}(\mathbf{X}, \hat{\mathbf{X}}) = \frac{1}{N \times T_{\text{out}}} \sum_{t=1}^{T_{\text{out}}} \sum_{n=1}^{N} \frac{|x_{t,n} - \hat{x}_{t,n}|}{(|x_{t,n}| + |\hat{x}_{t,n}|) / 2}
\end{equation}

\subsection{Numerical Stability}
\label{app:sec: numerical stability}

Given that \framework utilizes an ODE solver to model continuous dynamics and incorporates complex spatiotemporal dependencies, it is necessary to verify the model's numerical stability. The training loss curve over 100 epochs (Figure~\ref{fig:training_loss}) demonstrates that the model achieves stable convergence. Besides, our model incorporates robust design elements, such as normalization techniques, which significantly contributes to numerical stability during the optimization process.
\begin{figure}[t]
    \centering
    \small
    \begin{tikzpicture}
        \begin{axis}[
            width=0.6\linewidth,
            height=5cm,
            xlabel={Epoch},
            ylabel={Training Loss},
            xmin=1,
            xmax=100,
            grid=major,
            grid style={dashed, gray!30},
            axis line style={gray!80},
            tick align=outside,
            tick pos=left,
            legend style={
                at={(0.97,0.97)},
                anchor=north east,
                draw=none
            }
        ]
        \addplot[
            blue,
            thick,
            no markers
        ]
        table[
            x=epoch,
            y=train_loss,
            col sep=comma,
            header=has colnames
        ] {data/train_metrics.txt};
        \addlegendentry{Train Loss}
        \end{axis}
    \end{tikzpicture}
    \caption{The training curves on \textbf{KnowAir} datasets experimentally demonstrate that \framework achieves convergence.}
    \label{fig:training_loss}
\end{figure}

\begin{figure*}[t]
    \centering

    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/sudden_changes/sudden_change_case_3.png}
        \label{fig:sudden_up_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/sudden_changes/sudden_change_case_2.png}
        \label{fig:sudden_up_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/sudden_changes/sudden_change_case_1.png}
        \label{fig:sudden_down_1}
    \end{subfigure}

    \caption{Visualization results of \framework under sudden change on Hanoi dataset.}
    \label{fig:sudden_change_vis}
\end{figure*}


\subsection{Visualization of Sudden Change's Result}
\label{app:sec: sudden change}

To validate whether \framework can predict upward or downward trends during sudden changes (as described in Section~\ref{sec:experiments}), we visualize sudden changes at specific stations in \textbf{HanoiAir}, as shown in Figure~\ref{fig:sudden_change_vis}. In some cases, such as those illustrated, the peak pollutant concentrations are not well predicted. Although \framework outperforms other methods in the quantitative analysis of sudden change prediction, as shown in Table~\ref{tab:hanoi_results}, predicting sudden changes remains a significant challenge.


\section{More Experiment Results}
\label{app:sec: more_exp}
To scrutinize the temporal stability, we evaluate MAE at distinct forecasting steps ($t \in \{1, 3, \dots, 30\}$) in Table~\ref{tab:dynamic_spacing_mae}. While data-driven baselines excel in immediate steps via local fitting, their accuracy degrades rapidly as the horizon extends. In contrast, \framework{} resists error accumulation, outperforming PatchTST at the 9th step, validates that the Neural Kalman Fusion effectively mitigates the trajectory drift inherent in open-loop decoding.

\begin{table}[t]
\centering
\footnotesize
\caption{MAE comparison under dynamically time window forecasting horizons on \textbf{KnowAir} datasets.}
\label{tab:dynamic_spacing_mae}
\begin{tabular}{c | ccccc} 
\toprule
Model & 1st & 3rd & 9th & 18th & 30th \\
\midrule
\texttt{PatchTST}
& 7.13    & 12.82    & 24.11    & 25.56     & 26.14 \\
\texttt{S-Mamba}
& 7.54    & 10.06    & 26.37    & 25.85     & 25.88 \\
\texttt{Air-DualODE}
& 10.34   & 16.43    & 28.26    & 31.43     & 34.06 \\
\framework
& 7.67 & 11.06 & 16.48 & 21.10 & 24.65 \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Case study}
\subsubsection{Meteorology-Gated Neural Reaction}
To validate the interpretability and robustness of \framework, we go beyond standard metrics to analyze the internal mechanisms of the model. We specifically examine two critical aspects: the learning of chemical kinetics and the stability of long-term forecasting.

We first investigate the global behavior of the learned kinetics gate $\sigma(\mathcal{M}_t)$ across the entire test set. Figure~\ref{fig:case_study_1} presents the Kernel Density Estimation (KDE) of the gate activation values against ground-truth solar radiation.
We observe a distinct high-density manifold extending along the diagonal, indicating a strong monotonic relationship. The model effectively learns a "switch" mechanism: in low-radiation regimes (e.g., night or overcast), the gate remains closed ($\sigma \approx 0$), suppressing spurious reaction terms. Conversely, high radiation triggers gate activation ($\sigma \to 1$). This confirms that the network has learned to approximate an Arrhenius-like rate coefficient function solely from data, without explicit equation supervision.

To examine the dynamic impact of this gating mechanism, Figure~\ref{fig:case_study_1} visualizes a specific high-ozone episode. The temporal dynamics reveal a coherent photochemical process:
\begin{enumerate}
    \item \textit{Triggering:} As solar radiation peaks at noon (Bottom Panel), the Neural Gate synchronously opens, allowing the reaction term to contribute to the UDE drift.
    \item \textit{Consumption:} Coinciding with the gate opening, we observe a depletion in precursor $NO_2$ concentrations (Middle Panel), consistent with the photolysis reaction $NO_2 + h\nu \to NO + O$.
    \item \textit{Formation:} Consequently, the predicted $O_3$ concentration (Top Panel) rises sharply, accurately capturing the diurnal peak that baseline models often miss.
\end{enumerate}
This causal chain demonstrates that \framework does not merely memorize statistical correlations but simulates the underlying chemical kinetics, ensuring physical consistency in secondary pollutant forecasting.

\begin{figure}[t]
    \centering
    \footnotesize
    % --- Subfigure a: Chemical Dynamics (Dual Axis) ---
    \begin{subfigure}[b]{1.0\linewidth}
        \begin{tikzpicture}
            % TRỤC TRÁI: Ozone (O3) - Thang đo 150-325
            \begin{axis}[
                xlabel = Time (hours),
                ylabel = \textcolor{red}{Ozone ($O_3$) [$\mu g/m^3$]},
                axis y line*=left,      % Chỉ hiện trục Y bên trái
                ymin=120, ymax=350,     % Thang đo riêng cho O3
                width=1.0\linewidth,
                height=0.4\linewidth,   % Tăng chiều cao chút để dễ nhìn
                grid=major,
                grid style={dashed, gray!30},
                ylabel style={red, font=\bfseries},
                y tick label style={red},
                legend style={at={(0.25, 1.15)}, anchor=south, draw=none, fill=none}
            ]
                % Đường Ozone (TS_1) - Màu Đỏ
                \addplot[red, thick, mark=none] table[x=time, y=TS_1] {data/case_study_data.txt};
                \addlegendentry{Ozone ($O_3$) [$\mu g/m^3$]}
            \end{axis}

            % TRỤC PHẢI: NO2 (Precursor) - Thang đo 0-40
            \begin{axis}[
                % xlabel = Time (hours), % Không cần lặp lại nhãn X
                ylabel = \textcolor{blue}{Precursor ($NO_2$) [$\mu g/m^3$]},
                axis y line*=right,     % Chỉ hiện trục Y bên phải
                axis x line=none,       % Ẩn trục X (dùng chung với trục trái)
                ymin=0, ymax=60,        % Thang đo riêng cho NO2
                width=1.0\linewidth,
                height=0.4\linewidth,
                ylabel style={blue, font=\bfseries},
                y tick label style={blue},
                legend style={at={(0.75, 1.15)}, anchor=south, draw=none, fill=none}
            ]
                % Đường NO2 (TS_2) - Màu Xanh (Nét đứt để phân biệt)
                \addplot[blue, thick, mark=none] table[x=time, y=TS_2] {data/case_study_data.txt};
                \addlegendentry{Precursor ($NO_2$) [$\mu g/m^3$]}
            \end{axis}
        \end{tikzpicture}
        \vspace{5pt}
        \caption{Photochemical Dynamics: Inverse correlation between $O_3$ formation (Left Axis) and $NO_2$ consumption (Right Axis).}
        \label{subfig:o3-vs-no2}
    \end{subfigure}
    
    \vspace{10pt} % Khoảng cách giữa 2 biểu đồ
    
    % --- Subfigure b: Meteorological Catalyst ---
    \begin{subfigure}[b]{1.0\linewidth}
        \begin{tikzpicture}
            \begin{axis}[
                xlabel = Time (hours),
                ylabel = Radiation ($W/m^2$),
                ymin=0, 
                width=1.0\linewidth,
                height=0.35\linewidth,
                grid=major,
                grid style={dashed, gray!30},
                legend style={at={(0.5, 1.15)}, anchor=south, draw=none, fill=none},
                area style % Tô màu vùng dưới
            ]
                % Đường Radiation (TS_3) - Màu Cam
                \addplot[orange, thick, mark=none, fill=orange, fill opacity=0.2] table[x=time, y=TS_3] {data/case_study_data.txt};
                \addlegendentry{Solar Radiation}
            \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \caption{Meteorological Catalyst: Solar radiation intensity triggers the reaction.}
        \label{subfig:radiation}
    \end{subfigure}
    \begin{subfigure}[b]{1.0\linewidth}
    \centering
\includegraphics[width=0.75\linewidth]{images/KDE.png}
        \caption{Kernel Density Estimation of the learned Kinetics Gate activation versus ground-truth Solar Radiation}
        \label{subfig:kde}
    \end{subfigure}
    
    
    \caption{Visualization of the photochemical reaction mechanism. (a) The dual-axis plot clearly highlights that $O_3$ (red) peaks as $NO_2$ (blue) is depleted. (b) This process is synchronized with the solar radiation cycle.(c) Kernel Density Estimation of the learned Kinetics Gate activation versus ground-truth Solar Radiation. The high density along the diagonal confirms that the neural network explicitly learns to modulate reaction rates based on solar intensity, aligning with physical laws}
    \label{fig:case_study_1}
\end{figure}



\subsubsection{Diffusion and Advection}

To validate the physical fidelity of the UDE Process Model, Figure~\ref{fig:pm25_advection} visualizes the spatial evolution of the predicted PM$_{2.5}$ field alongside the dominant wind vectors. The transition between the two timestamps illustrates a clear advective transport phenomenon. Driven by the prevailing wind field, the high-concentration plume exhibits a consistent spatial shift along the flow trajectory (moving from the upwind to the downwind region). This directional alignment confirms that \framework successfully internalizes the explicit Advection equation to govern pollutant propagation, rather than merely treating wind as a static auxiliary feature.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/before.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/after.png}
    \end{subfigure}

    \caption{Visualization of predicted PM$_{2.5}$ concentrations under advection. The heatmap shows PM$_{2.5}$ concentration, while arrows represent wind direction.}
    \label{fig:pm25_advection}
\end{figure}


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented \framework, a novel framework that bridges the gap between data-driven efficiency and physical consistency for long-term air quality forecasting. By integrating a Universal Differential Equation governing transport-reaction dynamics with a Mamba-based measurement model via a \textit{closed-loop Neural Kalman Fusion}, \framework effectively mitigates the trajectory drift inherent in traditional open-loop solvers. Empirical evaluations on the different datasets demonstrate that our approach establishes promising results in prediction stability, significantly reducing long-term erors. 
These findings underscore the potential of assimilating domain knowledge—specifically chemical laws and mass conservation—into deep learning architectures for modeling chaotic environmental systems. For future work, we plan to extend this paradigm to graph-based multi-species interaction modeling to capture the full spectrum of atmospheric chemistry and explore probabilistic risk assessment for environmental policy-making.

==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Experimental Settings}
\paragraph{Datasets.} We evaluate \framework on two comprehensive, real-world air quality datasets: \textbf{KnowAir} and \textbf{HanoiAir}. Both datasets provide multi-year, hourly data crucial for modeling complex atmospheric dynamics, including secondary pollutant formation.

\textbf{KnowAir:} \footnote{\url{https://github.com/shuowang-ai/PM2.5-GNN}} 
This dataset covers the national-wide region (355 monitoring stations across the Beijing-Tianjin-Hebei with Surrounding Areas (BTHSA) and Yangtze River Delta (YRD), 70,128 hours from 2016-2023) \footnote{\url{https://www.mee.gov.cn/gkml/sthjbgw/qt/201701/t20170124_395229.htm}}. It integrates hourly Air Quality (AQ: PM\textsubscript{2.5}, O\textsubscript{3}), Meteorology \footnote{\url{https://cds.climate.copernicus.eu/datasets/reanalysis-era5-single-levels}} (Meteo: 8 variables), and importantly, gridded Emission inventories (Emi: NO\textsubscript{x}, VOC, SO\textsubscript{2}, NH\textsubscript{3}, PM\textsubscript{2.5}) derived from MEIC \footnote{\url{http://meicmodel.org.cn/}}.

\textbf{HanoiAir:} To assess generalizability, we construct a new dataset covering northern Vietnam (27 stations, approx. 70,128 hours from 2018-2025). This dataset contains hourly AQ measurements (PM\textsubscript{2.5}, O\textsubscript{3}, PM\textsubscript{10}, NO\textsubscript{x}, SO\textsubscript{2}, CO) and Meteo variables (6 vars). It also incorporates corresponding hourly-downscaled emission data (NO\textsubscript{x}, VOC, SO\textsubscript{2}, NH\textsubscript{3}, PM\textsubscript{2.5}) processed using standardized methodologies referenced in related works. Further details are provided in Appendix~\ref{app:hanoiair}.

For both datasets, we employ a chronological split to evaluate the model's forecasting ability on unseen future data. With \textbf{KnowAir}, We use 2016-2019 for training, 2020-2021 for validation, and 2022-2023 for testing. For \textbf{HanoiAir}, we adopt a similar chronological split: 2018-2021 for training, 2022-2023 for validation, and 2024-2025 for testing.

\paragraph{Baselines.}
We compare \framework against a diverse set of baseline models spanning several categories:
\begin{itemize}
    \item \textbf{Statistical Methods:} Standard time series models including \texttt{HA} (Historical Average) and \texttt{VAR} (Vector Autoregression)~\cite{DBLP:journals/tsp/ZamanLRB21}.
    \item \textbf{Neural ODE / Physics-Informed Models:} Methods incorporating differential equations or physics principles, such as \texttt{LatentODE}~\cite{DBLP:conf/nips/ChenRBD18}, \texttt{ODE-LSTM}~\cite{DBLP:journals/corr/abs-2006-04418}, \texttt{Air-DualODE}~\cite{DBLP:conf/iclr/TianL0CGZPRY25}, and \texttt{AirPhyNet}~\cite{DBLP:conf/iclr/HettigeJXLCW24}.
    \item \textbf{GNN-based Spatio-Temporal Models:} Models explicitly designed for graph-structured time series data, including \texttt{STGCN}~\cite{DBLP:conf/ijcai/YuYZ18}, \texttt{DCRNN}~\cite{DBLP:conf/iclr/LiYS018}, \texttt{GTS}~\cite{DBLP:conf/iclr/Shang0B21}, and \texttt{PM25GNN}~\cite{DBLP:conf/gis/WangLZMMG20}.
    \item \textbf{Linear and MLP-based Models:} Recent efficient architectures focusing on simpler mappings, such as \texttt{DLinear}~\cite{DBLP:conf/aaai/ZengCZ023} and \texttt{ModernTCN}~\cite{DBLP:journals/corr/abs-1803-01271}).
    \item \textbf{Transformer-based Models:} Models leveraging attention mechanisms, including \texttt{Fredformer}~\cite{DBLP:conf/kdd/Piao0MMS24}, \texttt{PatchTST}~\cite{DBLP:conf/iclr/NieNSK23}, \texttt{Crossformer}~\cite{DBLP:conf/iclr/ZhangY23}, and \texttt{TimeMoE}~\cite{DBLP:conf/iclr/ShiWNLYWJ25}.
    \item \textbf{State Space Models (SSMs):} Models based on structured state space representations, such as \texttt{SMamba} (based on Mamba~\cite{DBLP:journals/corr/abs-2312-00752}), \texttt{S4}~\cite{DBLP:conf/iclr/GuGR22}, and \texttt{BiMamba}~\cite{DBLP:journals/corr/abs-2411-11843}.
\end{itemize}

\paragraph{Metrics.}
To quantitatively assess the performance of \framework and baseline models, we employ three standard forecasting metrics: Mean Absolute Error (MAE), Root Mean Square Error (RMSE), and Symmetric Mean Absolute Percentage Error (SMAPE). Formal definitions of these metrics are provided in Appendix~\ref{app:metrics}.

\paragraph{Hyperparameter Settings.}
We train \framework using AdamW~\cite{DBLP:conf/iclr/LoshchilovH19} optimizer with a learning rate of 0.00001 and a batch size of 64. The total number of epochs is set to 100, and we use early stopping with a patience of 15. 

\paragraph{Implementation Details.}
We implement \framework and baselines using Python 3.12, Numpy 2.3.3, SciPy 1.15.3, Sklearn 1.7.2, and Pytorch 2.8.0. We run all experiments on a cluster server, which runs Ubuntu Linux 22.04 LTS. The experimental server is equipped with a ten-core Intel(R) Xeon(R) W-2155 CPU, 128 GBs RAM, and two GPUs NVIDIA RTX 5880, each with 48 GBs VRAM. 
% We made the source code publicly available at \underline{\url{https://github.com/kiendemo/AeroChem}}.


\paragraph{Forecasting Scenarios.} We evaluate these metrics across multiple forecasting horizons to assess both short-term and longer-term predictive capabilities. Specifically, performance is reported for average errors over forecast windows of \textbf{3 days} (1-72 hours), \textbf{6 days} (1-144 hours), \textbf{9 days} (1-216 hours) and \textbf{Sudden Change} events~\cite{DBLP:conf/iclr/TianL0CGZPRY25}, these events are identified as time steps where the ground-truth PM\textsubscript{2.5} concentration exceeds 75 $\mu\text{g}/\text{m}^3$ and subsequently fluctuates by more than ±20 $\mu\text{g}/\text{m}^3$ within the next three hours. The metrics are calculated exclusively on these identified sudden change instances within the test set. All metrics are computed on the predictions after inverse-transforming them back to the original physical scale (e.g., $\mu\text{g}/\text{m}^3$) and are reported for both the \textbf{KnowAir} and \textbf{HanoiAir} datasets.

\subsection{Main results}

Tables~\ref{tab:know_results} and~\ref{tab:hanoi_results} present the experimental results on the \textbf{KnowAir} and \textbf{HanoiAir} datasets. Overall, \framework achieves the best performance in most cases, significantly outperforming state-of-the-art baselines across different forecasting horizons and metrics. The results reveal the following key observations:

First, \framework effectively mitigates long-term error accumulation. While Transformer-based models (e.g., \texttt{TimeMoE}, \texttt{PatchTST}) exhibit competitive short-term accuracy due to strong local fitting, their performance deteriorates significantly as the horizon extends. In contrast, \framework maintains robust stability. On the KnowAir dataset (9-day horizon), it surpasses the strongest baseline (\texttt{TimeMoE}) by a margin of 4.9\% in MAE and 2.0\% in RMSE. This superiority is attributed to the Physics-informed Process Model (UDE), which acts as a continuous physical regularizer to constrain the latent trajectory, thereby preventing the drift inherent in open-loop decoding.

Second, \framework exhibits superior robustness in noisy, data-scarce environments. The performance gap widens on the HanoiAir dataset, which is characterized by higher sparsity and noise. In this setting, \framework achieves the lowest errors, outperforming \texttt{TimeMoE} by 6.1\% in 9-day MAE. This indicates that the Neural Kalman Fusion module plays a critical role in filtering measurement noise and correcting state variance, making the framework significantly more robust than direct mapping approaches when facing high-entropy data.

Third, \framework demonstrates sensitivity to sudden pollution events. Existing methods tend to over-smooth abrupt changes towards the mean. As evidenced in the ``Sudden Change'' evaluation, \framework yields substantial improvements, reducing MAE by 5.6\% compared to \texttt{TimeMoE} and 13.4\% compared to S-Mamba. This gain stems from the Meteorology-gated Neural Reaction mechanism. By explicitly modeling non-linear chemical kinetics triggered by environmental drivers (e.g., radiation, temperature), the model anticipates rapid secondary pollutant formation that historical autocorrelation alone fails to capture.

\input{tables/knowair-all-overall}

Fig.~\ref{fig:horizon_analysis} illustrates the error evolution across varying horizons. \framework exhibits superior stability compared to existing physics-guided baselines (e.g., \texttt{AirPhyNet}, \texttt{Air-DualODE}), with the performance gap widening significantly as the prediction window extends. While prior methods suffer from rapid error propagation, \framework maintains a flattened error trajectory, validating the effectiveness of our closed-loop design in mitigating long-term physical drift.


\subsection{Ablation Study}
\label{sec:ablation}

We study the effectiveness of each component in the proposed framework by iteratively removing components in an ablation study on the \textbf{KnowAir} and \textbf{HanoiAir} datasets. We categorize the variants into two groups: (1) \textit{Physical Mechanism Analysis}, which validates the explicit process modeling components, and (2) \textit{Architecture Analysis}, which assesses the data-driven backbone and the fusion strategy.

\paragraph{Effect of Physical Mechanisms.}
\label{sec:ablation_physics}

We first investigate the effectiveness of the physics-informed drift function in the Process Model defined in Eq.~\ref{eq:ude_master} by removing components. Specifically, we remove the isotropic diffusion (\framework{\texttt{-D}}), the anisotropic advection (\framework{\texttt{-A}}), meteorology-gated neural reaction module (\framework{\texttt{-R}}), remove all explicit physical terms (\framework{\texttt{-P}}).

Removing physical guidance (\textit{-P}) leads to severe long-term degradation (MAE increases by \textbf{20.8\%} on KnowAir), confirming the UDE's role in preventing trajectory drift. Notably, the Reaction module (\textit{-R}) dominates the performance contribution, surpassing transport dynamics (\textit{-A}, \textit{-D}). This validates that explicitly modeling meteorology-driven chemical kinetics is critical for capturing secondary pollutant formation, a feature missing in pure advection-diffusion baselines.

\input{tables/hanoiair-all-overall}


\input{tables/fig_horizon_errors}




\paragraph{Effect of Models and Fusion}
\label{sec:ablation_arch}

Next, we evaluate the contributions of the \textbf{S-Mamba} backbone on the Measurement Model and the \textbf{Neural Kalman Fusion} mechanism on KnowAir dataset.
\begin{itemize}
    \item \framework{\textit{-M}}: We replace the S-Mamba encoder with a standard Bi-directional LSTM to evaluate the capability of capturing long-range temporal dependencies.
    \item \framework{\textit{-K}}: We remove the recursive correction step defined in Eq.~\ref{eq:posterior}. The prior state $\mathbf{S}^-_t$ is directly used as the input for the next step ($\mathbf{S}^+_t \leftarrow \mathbf{S}^-_t$), degrading the model to an open-loop UDE solver.
    \item \framework{\textit{-N}}: We retain the standard Kalman update but remove the learnable correction term ($\boldsymbol{\epsilon}'_t = \boldsymbol{\epsilon}_t$). This assumes the residuals follow a strictly Gaussian distribution.
    \item \textit{\textbf{Late Fusion}}: We decouple the Process and Measurement Model to operate independently without latent interaction. Their outputs are decoded separately into the explicit space and combined via weighted averaging.
\end{itemize}

The open-loop variant (\textit{-K}) suffers a catastrophic failure (MAE +47.4\%), identifying the Neural Kalman Fusion as the absolute core driver of system stability. Regarding the backbone, replacing S-Mamba with Bi-LSTM (\textit{-M}) causes significant accuracy loss at the 9-day horizon, proving Mamba's superiority in modeling global temporal dependencies. Finally, the inferiority of \textit{Late Fusion} confirms that deep latent assimilation is strictly required over shallow ensembling to correct physical states.


\input{tables/ablation}


\subsection{Parameter Studies}
\label{sec:sensitivity}

We assess the model's robustness to three key hyperparameters (Fig.~\ref{fig:sensitivity}).

\textit{\textbf{Physics Weight ($\lambda_{\text{phy}}$):}} Fig.~\ref{fig:sens_phy} reveals a distinct trade-off between physical constraints and data flexibility, forming a bell-shaped performance curve. With negligible regularization ($\lambda_{phy} \to 0$), the model degenerates into a purely data-driven solver, suffering from higher errors due to the lack of guidance against long-term drift. Conversely, excessive regularization ($\lambda_{phy} > 1$) forces the latent states to strictly adhere to simplified dynamics, rendering the model too rigid to capture complex, localized variations. The performance peaks at $\lambda_{phy} = 0.1$, confirming this as the optimal equilibrium where physical laws stabilize the trajectory without suppressing the data-driven backbone's adaptability.

\textit{\textbf{Model Dimension ($d_{\text{model}}$):}} As depicted in Fig~\ref{fig:sens_dim}, expanding the hidden dimension initially yields substantial gains, confirming that sufficient representational capacity is requisite for encoding complex spatiotemporal dependencies. However, performance saturates beyond $d_{\text{model}}=96$, where further increases offer negligible improvements while inflating computational costs. Consequently, we select 96 as the optimal equilibrium between model expressiveness and computational efficiency.

\textit{\textbf{Solver Step ($dt$):}} Figure~\ref{fig:sens_dt} demonstrates the model's remarkable numerical robustness, maintaining consistent accuracy across varying step sizes. Typically, coarser discretization introduces integration errors in standard ODE solvers. However, our results indicate that the fusion mechanism effectively rectifies these trajectory deviations by assimilating data-driven corrections.

\begin{figure*}[t]
    \centering
    % Thiết lập style chung cho đẹp
    \pgfplotsset{
        every axis/.style={
            width=\linewidth,
            height=5cm,
            grid=major,
            grid style={dashed,gray!30},
            xlabel near ticks,
            ylabel near ticks,
            label style={font=\footnotesize},
            tick label style={font=\footnotesize},
            legend style={
                at={(0.5,1.15)}, 
                anchor=south, 
                legend columns=-1,
                draw=none, 
                font=\footnotesize,
                fill=none
            },
            mark size=2pt
        }
    }

    % --- Subfigure 1: Physics Weight ---
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Physics Weight ($\lambda_{\text{phy}}$)},
                ylabel={Error},
                xmin=0, xmax=1.05,
                xtick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
                % Dùng semilogx nếu muốn nhìn rõ vùng 0.0-0.1, nhưng linear dễ so sánh tổng thể
            ]
            
            % MAE Line (Blue, Circle)
            \addplot[color=blue, mark=*, thick] coordinates {
                (0.0, 25.65) (0.005, 25.24) (0.01, 24.97) (0.02, 24.63) 
                (0.05, 24.20) (0.1, 24.08) (0.2, 24.22) (0.5, 24.74) (1.0, 25.25)
            };
            \addlegendentry{MAE}

            % RMSE Line (Red, Square)
            \addplot[color=red, mark=square*, thick] coordinates {
                (0.0, 41.48) (0.005, 40.86) (0.01, 40.47) (0.02, 40.00) 
                (0.05, 39.48) (0.1, 39.34) (0.2, 39.50) (0.5, 40.07) (1.0, 40.63)
            };
            \addlegendentry{RMSE}
            
            % Highlight Sweet Spot
            \draw[dashed, black!60] (axis cs:0.1, 20) -- (axis cs:0.1, 42);
            \end{axis}
        \end{tikzpicture}
        \caption{Effect of Physics Weight ($\lambda_{\text{phy}}$)}
        \label{fig:sens_phy}
    \end{subfigure}
    \hfill
    % --- Subfigure 2: Model Dimension ---
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Model Dimension ($d_{\text{model}}$)},
                % ylabel={Error}, % Bỏ ylabel giữa cho đỡ rối
                xtick={64, 96, 128},
                xmin=50, xmax=140,
            ]
            \addplot[color=blue, mark=*, thick] coordinates {
                (64, 25.30) (96, 24.08) (128, 24.50)
            };
            \addlegendentry{MAE}

            \addplot[color=red, mark=square*, thick] coordinates {
                (64, 40.06) (96, 39.34) (128, 39.66)
            };
            \addlegendentry{RMSE}
            
            \draw[dashed, black!60] (axis cs:96, 20) -- (axis cs:96, 42);
            \end{axis}
        \end{tikzpicture}
        \caption{Effect of Dimension ($d_{\text{model}}$)}
        \label{fig:sens_dim}
    \end{subfigure}
    \hfill
    % --- Subfigure 3: Solver Step ---
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Solver Step ($dt$)},
                % ylabel={Error},
                xmin=0, xmax=2.2,
                xtick={0.25, 0.5, 1.0, 1.5, 2.0},
            ]
            \addplot[color=blue, mark=*, thick] coordinates {
                (0.25, 33.22) (0.5, 27.88) (0.75, 25.01) 
                (1.0, 24.08) (1.25, 27.40) (1.5, 37.52) (2.0, 54.87)
            };
            \addlegendentry{MAE}

            \addplot[color=red, mark=square*, thick] coordinates {
                (0.25, 49.14) (0.5, 45.35) (0.75, 41.08) 
                (1.0, 39.34) (1.25, 43.92) (1.5, 57.84) (2.0, 81.46)
            };
            \addlegendentry{RMSE}
            
            \draw[dashed, black!60] (axis cs:1.0, 20) -- (axis cs:1.0, 85);
            \end{axis}
        \end{tikzpicture}
        \caption{Effect of Solver Step ($dt$)}
        \label{fig:sens_dt}
    \end{subfigure}

    \caption{Sensitivity analysis on KnowAir dataset. The dashed vertical lines indicate the default hyperparameters used in the full model ($\lambda=0.1, d=96, dt=1.0$), which consistently correspond to the optimal performance regions (lowest error).}
    \label{fig:sensitivity}
\end{figure*}


\subsection{Case study}
\subsubsection{Meteorology-Gated Neural Reaction}
To validate the interpretability and robustness of \framework, we go beyond standard metrics to analyze the internal mechanisms of the model. We specifically examine two critical aspects: the learning of chemical kinetics and the stability of long-term forecasting.

We first investigate the global behavior of the learned kinetics gate $\sigma(\mathcal{M}_t)$ across the entire test set. Figure~\ref{fig:case_study_1} presents the Kernel Density Estimation (KDE) of the gate activation values against ground-truth solar radiation.
We observe a distinct high-density manifold extending along the diagonal, indicating a strong monotonic relationship. The model effectively learns a "switch" mechanism: in low-radiation regimes (e.g., night or overcast), the gate remains closed ($\sigma \approx 0$), suppressing spurious reaction terms. Conversely, high radiation triggers gate activation ($\sigma \to 1$). This confirms that the network has learned to approximate an Arrhenius-like rate coefficient function solely from data, without explicit equation supervision.

To examine the dynamic impact of this gating mechanism, Figure~\ref{fig:case_study_1} visualizes a specific high-ozone episode. The temporal dynamics reveal a coherent photochemical process:
\begin{enumerate}
    \item \textit{Triggering:} As solar radiation peaks at noon (Bottom Panel), the Neural Gate synchronously opens, allowing the reaction term to contribute to the UDE drift.
    \item \textit{Consumption:} Coinciding with the gate opening, we observe a depletion in precursor $NO_2$ concentrations (Middle Panel), consistent with the photolysis reaction $NO_2 + h\nu \to NO + O$.
    \item \textit{Formation:} Consequently, the predicted $O_3$ concentration (Top Panel) rises sharply, accurately capturing the diurnal peak that baseline models often miss.
\end{enumerate}
This causal chain demonstrates that \framework does not merely memorize statistical correlations but simulates the underlying chemical kinetics, ensuring physical consistency in secondary pollutant forecasting.

\begin{figure}[t]
    \centering
    \footnotesize
    % --- Subfigure a: Chemical Dynamics (Dual Axis) ---
    \begin{subfigure}[b]{1.0\linewidth}
        \begin{tikzpicture}
            % TRỤC TRÁI: Ozone (O3) - Thang đo 150-325
            \begin{axis}[
                xlabel = Time (hours),
                ylabel = \textcolor{red}{Ozone ($O_3$) [$\mu g/m^3$]},
                axis y line*=left,      % Chỉ hiện trục Y bên trái
                ymin=120, ymax=350,     % Thang đo riêng cho O3
                width=1.0\linewidth,
                height=0.4\linewidth,   % Tăng chiều cao chút để dễ nhìn
                grid=major,
                grid style={dashed, gray!30},
                ylabel style={red, font=\bfseries},
                y tick label style={red},
                legend style={at={(0.25, 1.15)}, anchor=south, draw=none, fill=none}
            ]
                % Đường Ozone (TS_1) - Màu Đỏ
                \addplot[red, thick, mark=none] table[x=time, y=TS_1] {data/case_study_data.txt};
                \addlegendentry{Ozone ($O_3$) [$\mu g/m^3$]}
            \end{axis}

            % TRỤC PHẢI: NO2 (Precursor) - Thang đo 0-40
            \begin{axis}[
                % xlabel = Time (hours), % Không cần lặp lại nhãn X
                ylabel = \textcolor{blue}{Precursor ($NO_2$) [$\mu g/m^3$]},
                axis y line*=right,     % Chỉ hiện trục Y bên phải
                axis x line=none,       % Ẩn trục X (dùng chung với trục trái)
                ymin=0, ymax=60,        % Thang đo riêng cho NO2
                width=1.0\linewidth,
                height=0.4\linewidth,
                ylabel style={blue, font=\bfseries},
                y tick label style={blue},
                legend style={at={(0.75, 1.15)}, anchor=south, draw=none, fill=none}
            ]
                % Đường NO2 (TS_2) - Màu Xanh (Nét đứt để phân biệt)
                \addplot[blue, thick, mark=none] table[x=time, y=TS_2] {data/case_study_data.txt};
                \addlegendentry{Precursor ($NO_2$) [$\mu g/m^3$]}
            \end{axis}
        \end{tikzpicture}
        \vspace{5pt}
        \caption{Photochemical Dynamics: Inverse correlation between $O_3$ formation (Left Axis) and $NO_2$ consumption (Right Axis).}
        \label{subfig:o3-vs-no2}
    \end{subfigure}
    
    \vspace{10pt} % Khoảng cách giữa 2 biểu đồ
    
    % --- Subfigure b: Meteorological Catalyst ---
    \begin{subfigure}[b]{1.0\linewidth}
        \begin{tikzpicture}
            \begin{axis}[
                xlabel = Time (hours),
                ylabel = Radiation ($W/m^2$),
                ymin=0, 
                width=1.0\linewidth,
                height=0.35\linewidth,
                grid=major,
                grid style={dashed, gray!30},
                legend style={at={(0.5, 1.15)}, anchor=south, draw=none, fill=none},
                area style % Tô màu vùng dưới
            ]
                % Đường Radiation (TS_3) - Màu Cam
                \addplot[orange, thick, mark=none, fill=orange, fill opacity=0.2] table[x=time, y=TS_3] {data/case_study_data.txt};
                \addlegendentry{Solar Radiation}
            \end{axis}
        \end{tikzpicture}
        \vspace{-5pt}
        \caption{Meteorological Catalyst: Solar radiation intensity triggers the reaction.}
        \label{subfig:radiation}
    \end{subfigure}
    \begin{subfigure}[b]{1.0\linewidth}
    \centering
\includegraphics[width=0.75\linewidth]{images/KDE.png}
        \caption{Kernel Density Estimation of the learned Kinetics Gate activation versus ground-truth Solar Radiation}
        \label{subfig:kde}
    \end{subfigure}
    
    
    \caption{Visualization of the photochemical reaction mechanism. (a) The dual-axis plot clearly highlights that $O_3$ (red) peaks as $NO_2$ (blue) is depleted. (b) This process is synchronized with the solar radiation cycle.(c) Kernel Density Estimation of the learned Kinetics Gate activation versus ground-truth Solar Radiation. The high density along the diagonal confirms that the neural network explicitly learns to modulate reaction rates based on solar intensity, aligning with physical laws}
    \label{fig:case_study_1}
\end{figure}



\subsubsection{Diffusion and Advection}

To validate the physical fidelity of the UDE Process Model, Figure~\ref{fig:pm25_advection} visualizes the spatial evolution of the predicted PM$_{2.5}$ field alongside the dominant wind vectors. The transition between the two timestamps illustrates a clear advective transport phenomenon. Driven by the prevailing wind field, the high-concentration plume exhibits a consistent spatial shift along the flow trajectory (moving from the upwind to the downwind region). This directional alignment confirms that \framework successfully internalizes the explicit Advection equation to govern pollutant propagation, rather than merely treating wind as a static auxiliary feature.

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/before.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/after.png}
    \end{subfigure}

    \caption{Visualization of predicted PM$_{2.5}$ concentrations under advection. The heatmap shows PM$_{2.5}$ concentration, while arrows represent wind direction.}
    \label{fig:pm25_advection}
\end{figure}





==> sections/introduction.tex <==
% \section{Introduction}
% \label{sec:introduction}


% \begin{figure}[t]
%     \centering    \includegraphics[width=0.95\columnwidth]{images/Air_pollutant.jpg}
%     \caption{An air quality modelling system simulates the key processes involved as pollutants move
% through the atmosphere.}
%     \label{fig:example}
% \end{figure}

% Air quality forecasting is a cornerstone of effective environmental policy and public health protection. The complex dynamics of atmospheric pollutants are traditionally modeled using two main paradigms: physics-based models, which simulate atmospheric processes but are computationally intensive, and data-driven models, which excel at pattern recognition but may yield physically implausible results. A promising frontier in recent years has been the development of physics-guided neural networks that seek to synergize these two approaches \citep{tian2025air}. However, existing hybrid models often face a critical trade-off: in striving for tractability, they tend to oversimplify the underlying physics, leaving significant gaps in their representation of real-world atmospheric phenomena. This paper identifies and addresses two fundamental limitations of current state-of-the-art models: the inadequate modeling of secondary pollutant chemistry and the failure to capture long-range temporal dependencies.

% The first and more subtle challenge lies in modeling the formation of \textbf{secondary pollutants}. A substantial fraction of the most hazardous pollutants, such as ground-level ozone ($O_3$) and fine particulate matter (PM$_{2.5}$), are not emitted directly. Instead, they are formed in the atmosphere through complex, non-linear chemical reactions of precursor gases (e.g., $NO_x$, $SO_2$, VOCs) under specific meteorological conditions. This chemical transformation is a central problem in atmospheric science, as secondary aerosols constitute a major component of PM$_{2.5}$ mass globally \citep{hallquist2009formation} and have been linked to higher health risks compared to primary emissions \citep{daellenbach2020sources}. Despite its importance, many contemporary physics-guided models \cite{hettige2024airphynet} \citep{tian2025air} primarily focus on the physics of transport (i.e., advection and diffusion). They often simplify chemical processes into linear source/sink correction terms, failing to capture the rich, non-linear dynamics of secondary pollutant formation. This omission represents a significant gap in faithfully modeling urban air pollution. More recent surrogate models, such as PCDCNet \citep{wang2025pcdcnet}, have made progress by incorporating emission data to learn these chemical interactions. However, this is typically achieved through implicit, 'black-box' modules like Multi-Layer Perceptrons (MLPs), which learn correlations from data but are not explicitly constrained by the fundamental structure of chemical kinetic equations. This lack of a strong physical inductive bias for the reaction process itself represents a significant gap in faithfully and robustly modeling urban air pollution.

% The second critical limitation is the reliance on \textbf{short-term historical context}. Many state-of-the-art forecasting models operate on a limited temporal window, typically 72 hours, to predict future concentrations \citep{tian2025air}. This narrow view fundamentally prevents the model from learning longer-timescale dynamics that are known to govern air quality. For instance, a 72-hour window is insufficient to capture the distinct weekly cycles in emissions resulting from human activity, a standard component of air quality data analysis \citep{carslaw2012openair}. Furthermore, severe pollution episodes are often driven by large-scale, synoptic meteorological patterns, such as slow-moving high-pressure systems, that evolve over several days to a week \citep{tai2010correlations}. Models with short-term memory can only observe the immediate effects of these patterns, not their formation and evolution, thus limiting their long-term predictive power. This challenge is widely recognized in the broader machine learning community as Long Sequence Time-Series Forecasting (LSTF), which requires specialized architectures beyond conventional models \citep{zhou2021informer}. Advanced frameworks like PCDCNet rely on recurrent architectures (GRUs) for temporal modeling, which have known limitations in capturing very long-range dependencies. This challenge is widely recognized in the broader machine learning community as Long Sequence Time-Series Forecasting (LSTF), which requires specialized architectures beyond conventional models \citep{zhou2021informer}.

% To address these dual challenges simultaneously, we propose \framework, a novel dual-branch, physics-informed framework for air quality forecasting. \framework\ is designed from the ground up to bridge the gaps left by previous models. It consists of two specialized, synergistic branches:
% \begin{enumerate}
%     \item A \textbf{Physics-Informed Dynamics Branch} that explicitly models the formation of secondary pollutants. It does so by incorporating a neural operator that approximates the solution of the full Advection-Diffusion-\textbf{Reaction} system of Partial Differential Equations (PDEs), capturing the non-linear chemical kinetics.
%     \item A \textbf{Data-Driven Dynamics Branch} that leverages a state-of-the-art State Space Model (SSM) architecture, Mamba, to efficiently process long historical sequences and capture the long-range temporal dependencies, such as weekly and seasonal patterns, that short-window models miss.
% \end{enumerate}
% These two branches are intelligently integrated through a gated fusion mechanism, allowing the model to produce forecasts that are both deeply informed by physical chemistry and accurately grounded in long-term data-driven patterns. In summary, our contributions are:
% \begin{itemize}
%     \item We identify and articulate two critical, concurrent limitations in state-of-the-art air quality forecasting models: the neglect of complex secondary pollutant chemistry and the inability to capture long-range temporal dependencies.
%     \item We propose \framework, a novel dual-branch architecture that is the first to synergistically combine a PDE-based chemical reaction model with a long-sequence State Space Model to address these limitations.
%     \item We demonstrate through extensive experiments that \framework\ achieves state-of-the-art performance, showing significant improvements in forecasting secondary pollutants and in long-horizon prediction scenarios where previous models falter.
% \end{itemize}

% The rest of this paper is organized as follows. Section~\ref{sec:preliminaries} introduces the formal problem definition. Section~\ref{sec:methodology} details the architecture of \framework. Experimental results are presented in Section~\ref{sec:experiments}, followed by related work in Section~\ref{sec:related-work} and our conclusion in Section~\ref{sec:conclusion}.


\section{Introduction}
\label{sec:introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{images/Air_pollutant.jpg}
    \caption{An illustration of the complex interplay between transport dynamics and chemical reactions in air quality modeling.}
    \label{fig:example}
\end{figure}

Air quality forecasting is a cornerstone of effective environmental policy and public health protection. The complex dynamics of atmospheric pollutants are traditionally modeled using two main paradigms: physics-based Chemical Transport Models (CTMs), which simulate atmospheric processes based on first principles but are computationally prohibitive, and data-driven Deep Learning (DL) models, which excel at pattern recognition but often yield physically implausible results. A promising frontier in recent years has been the development of \textit{Physics-Informed Machine Learning} (PIML) that seeks to synergize these two approaches \citep{tian2025air}. However, existing hybrid models often face a critical trade-off: in striving for tractability, they tend to oversimplify the underlying physics, leaving significant gaps in their representation of real-world atmospheric phenomena.                                                        
This paper identifies and addresses two fundamental limitations of current state-of-the-art models: the inadequate modeling of \textbf{secondary pollutant formation} and the lack of robustness in \textbf{long-term forecasting}.

The first and more subtle challenge lies in modeling the chemical kinetics of secondary pollutants. A substantial fraction of hazardous pollutants, such as ground-level ozone ($O_3$) and fine particulate matter (PM$_{2.5}$), are not emitted directly but formed through complex, non-linear photochemical reactions of precursors (e.g., $NO_x$, VOCs) under specific meteorological conditions \citep{hallquist2009formation, daellenbach2020sources}. Despite its importance, many contemporary physics-guided models primarily focus on transport physics (advection-diffusion) \citep{hettige2024airphynet, tian2025air}. They often reduce chemical processes to simplified linear source/sink terms or use generic 'black-box' Multi-Layer Perceptrons (MLPs) \citep{wang2025pcdcnet}. These approaches lack the strong \textit{inductive bias} required to model multiplicative chemical interactions (e.g., the Arrhenius law), leading to poor generalization in predicting secondary formation events.

The second critical limitation is the \textbf{error accumulation (drift)} in long-term forecasting. Current autoregressive models operate in an open-loop manner, where small prediction errors at early steps propagate and amplify over time \citep{zhou2021informer}. While advanced architectures like Transformers or State Space Models (e.g., Mamba) capture long-range dependencies that local differential operators usually miss, they lack a mechanism to strictly constrain the trajectory within physical bounds over long horizons. Purely physics-based solvers (ODEs), on the other hand, are sensitive to initial conditions and system noise, often diverging without continuous data correction. There is a lack of a unified framework that can simultaneously leverage the long-term memory of data-driven models and the stability of physical laws.

To address these dual challenges, we propose \framework, a novel closed-loop, physics-informed framework for air quality forecasting. Unlike previous loosely-coupled approaches, \framework integrates specialized components into a unified Data Assimilation system.

% \begin{enumerate}
%     \item A \textbf{Process Model} based on \textit{Universal Stochastic Differential Equations (UDEs)}. We explicitly decompose the dynamics into known physical transport (modeled by Graph Laplacian) and unknown chemical kinetics. Crucially, we introduce a \textbf{Meteo-Gated Neural Reaction} module that mimics the law of mass action, allowing the model to learn non-linear secondary formation rates driven by meteorological catalysts.
    
%     \item A \textbf{Measurement Model} utilizing \textbf{S-Mamba}, a selective State Space Model, to act as a "virtual sensor". It efficiently extracts global spatiotemporal contexts from long historical sequences to provide adaptive observations and uncertainty estimates.
    
%     \item A \textbf{Neural Kalman Fusion} mechanism that closes the loop. Instead of static fusion, we employ a recursive Kalman Filter to optimally assimilate the physics-based prior and data-driven measurement at each time step. The posterior state is fed back into the UDE, continuously correcting the trajectory to prevent long-term drift.
% \end{enumerate}

In summary, our contributions are:

\begin{itemize}
    \item We identify the limitations of current approaches in capturing complex chemical kinetics and preventing error accumulation in long-term forecasting. To address this, we propose \framework, a novel closed-loop framework that synergistically integrates Physics-informed Neural Network (PINN) with Neural Kalman Filtering.
    
    \item We design a specialized Reaction mechanism within the process model. This component explicitly models the non-linear formation of secondary pollutants based on meteorological conditions, bridging the gap between deep learning representations and fundamental physicochemical principles.
    
    \item We construct a newly compiled real-world dataset for Hanoi, Vietnam (HanoiAir), to evaluate the model's generalization capability in data-scarce regions. Extensive experiments on both the public KnowAir dataset and HanoiAir demonstrate that \framework showing significant improvements in forecasting secondary pollutants and maintaining stability over long horizons.
\end{itemize}

The rest of this paper is organized as follows. Section~\ref{sec:preliminaries} establishes the problem definition. Section~\ref{sec:methodology} details the \framework architecture. Experiments and results are presented in Section~\ref{sec:experiments}, followed by related work in Section~\ref{sec:related-work} and conclusion in Section~\ref{sec:conclusion}.

==> sections/methodology.tex <==
\section{Methodology}
\label{sec:methodology}

To address the probabilistic forecasting problem defined in Eq. \ref{eq:prob_forecasting_function}, specifically targeting the challenges of secondary pollutant formation and long-term stability, we propose \framework. Unlike previous hybrid frameworks that rely on loose coupling (e.g., parallel branches with simple gating), our model operates on the principle of \textit{Closed-loop Neural Data Assimilation}.

The architecture, illustrated in Figure~\ref{fig:framework_overview}, integrates three core components: (1) A \textbf{Measurement Model} utilizing S-Mamba to extract global temporal contexts; (2) A \textbf{Process Model} governed by a Universal Stochastic Differential Equation (UDE)\cite{DBLP:journals/corr/abs-2001-04385} to explicitly model transport and chemical kinetics; and (3) A \textbf{Neural Kalman Fusion} module that optimally assimilates these branches and recursively feeds the posterior state back into the physics engine.
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{images/Model.jpg}
    \caption{Overall \framework framework consists of the Measurement Model, the Process Model, and the Neural Kalman Fusion module. $\mathcal{R}_{t}$ represents the attention-based chemical reaction function . $\delta_{phy}$ represents the diffusion - advection function within the Universal Differential Equation (UDE).}
    \label{fig:framework_overview}
\end{figure*}

\subsection{Measurement Model: The Virtual Sensor}
The primary role of the Data Branch is to provide a robust "virtual observation" $\mathbf{Z}_{obs}$ and an associated uncertainty estimate $\mathbf{R}_{obs}$ derived from historical patterns. We employ \textbf{S-Mamba} \cite{DBLP:journals/ijon/WangKFWYZWZ25}, a selective state space model, to efficiently capture long-range dependencies from the historical sequence $\mathbf{X}_{1:T_{in}}$.

The S-Mamba encoder processes the sequence to extract a global context embedding $\mathbf{H}_{ctx} \in \mathbb{R}^{N \times d_{model}}$. To optimize computational efficiency for autoregressive decoding, we employ a static-dynamic decomposition strategy:

\begin{align}
    \mathbf{Z}_{base}, \mathbf{R}_{base} &= \text{ProjHeads}(\mathbf{H}_{ctx}) \\
    \mathbf{Z}_{obs, t} &= \mathbf{Z}_{base} + \alpha \cdot \tanh(\mathbf{S}^+_{t-1}) \label{eq:adaptive_meas} \\
    \mathbf{R}_{obs, t} &= \text{Softplus}(\mathbf{R}_{base}) \cdot (1 + \beta \frac{t}{T_{out}}) \label{eq:adaptive_unc}
\end{align}

where $\mathbf{S}^+_{t-1}$ is the posterior latent state from the previous timestep. Eq. \ref{eq:adaptive_meas} allows the measurement to dynamically adapt to the current trajectory, while Eq. \ref{eq:adaptive_unc} models the increasing epistemic uncertainty over the forecast horizon, reflecting the growing epistemic uncertainty as the forecast horizon expands.

\subsection{Process Model}
We formulate the temporal evolution of the latent state $\mathbf{S}(t)$ as a controlled physics-inspired operator. For notational convenience, the dynamics in matrix form $S_t \in \mathbb{R}^{N \times D}$ implies a set of coupled SDEs where the Wiener process $dW_t$ consists of independent components acting element-wise. This formulation explicitly disentangles physical transport from complex chemical transformations:

\begin{equation}
    d\mathbf{S}_t = \underbrace{\mathcal{F}_{drift}(\mathbf{S}_t, \mathbf{E}_t, \mathbf{M}_t)}_{\text{Deterministic Dynamics}} dt + \underbrace{g(\mathbf{S}_t)}_{\text{Diffusion}} d\mathbf{W}_t
    \label{eq:ude_master}
\end{equation}

The drift function $\mathcal{F}_{drift}$ is a composite of three distinct terms, each corresponding to a specific atmospheric process:

\subsubsection{Isotropic Diffusion}
We model the background dispersion of pollutants based on geographical proximity. Let $\mathbf{L}_{diff} \in \mathbb{R}^{N \times N}$ be the normalized Graph Laplacian \cite{DBLP:conf/iclr/KipfW17} derived from the static distance matrix. The Laplacian operator acts strictly on the spatial dimension ($N \times N$) and is broadcast across the feature dimension $D$. The diffusion drift is defined as:
\begin{equation}
    \delta_{diff} = -\lambda_1 \mathbf{L}_{diff} \mathbf{S}_t
\end{equation}
The negative sign ensures flux from high-concentration to low-concentration regions, adhering to Fick's laws.

\subsubsection{Anisotropic Advection}
To capture wind-driven transport, we construct a time-varying dynamic Laplacian $\mathbf{L}_{adv}(t)$. At each step, we project the wind vector $\vec{v}_t$ onto the edge direction vectors $\vec{e}_{ij}$ of the graph to compute dynamic edge weights:
\begin{equation}
    w_{ij}(t) = \text{ReLU}\left( \frac{\vec{v}_{i,t} \cdot \vec{e}_{ij}}{||\vec{v}_{i,t}||} \right) \cdot ||\vec{v}_{i,t}||
\end{equation}
Using these weights, we construct $\mathbf{L}_{adv}(t)$ and compute the advection drift $\delta_{adv} = -\lambda_2 \mathbf{L}_{adv}(t) \mathbf{S}_t$. This term explicitly models the directional flow of pollutants driven by meteorology.

\subsubsection{Meteo-Gated Neural Reaction (Chemical Kinetics)}
To model the non-linear formation of secondary pollutants (e.g., $NO_x \to O_3$), we introduce a \textbf{Gated Interaction Mechanism} inspired by the Arrhenius equation \cite{LI2024113375}. While classical kinetics follow the Law of Mass Action (polynomial interactions), we employ Self-Attention to learn a generalized interaction map, allowing the model to discover non-stoichiometric dependencies between latent precursors and target pollutants.
To explicitly operationalize the reactant interaction, we define the input features as $\mathbf{H}_{react} = \text{Concat}(\mathbf{S}_t, \mathbf{E}_t) \in \mathbb{R}^{N \times (D_s + D_e)}$. The Self-Attention mechanism computes the interaction dynamics as follows:
\begin{equation}
    \mathbf{Q} = \mathbf{H}_{react}\mathbf{W}_Q, \quad \mathbf{K} = \mathbf{H}_{react}\mathbf{W}_K, \quad \mathbf{V} = \mathbf{H}_{react}\mathbf{W}_V
\end{equation}
where $\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V$ are learnable projection matrices. 
\textbf{Chemical Interpretation:} In this latent representation, $\mathbf{Q}$ (Queries) and $\mathbf{K}$ (Keys) encode the physicochemical properties of the reactants. Their dot product $\text{Softmax}(\frac{\mathbf{Q}\mathbf{K}^T}{\sqrt{d}})$ represents the learned \textit{affinity matrix}, approximating the collision probability between different latent species (e.g., matching precursors like $NO_x$ with conditions conducive to reaction). The $\mathbf{V}$ (Values) represents the potential magnitude of the chemical transformation resulting from these collisions.


This module takes reactants (State $\mathbf{S}_t$, Emissions $\mathbf{E}_t$) and environmental conditions (Scalar Meteorology $\mathbf{M}^{sc}_t$) as inputs:
\begin{equation}
    \mathcal{R}_{chem} = \underbrace{\text{Attn}(\mathbf{S}_t, \mathbf{E}_t)}_{\text{Reactant Interaction}} \odot \underbrace{\sigma(\text{MLP}(\mathbf{M}^{sc}_t))}_{\text{Kinetics Modulation Gate}}
\end{equation}
Here, $\odot$ denotes the element-wise product. This element-wise gating mechanism structurally enforces the requirement that chemical reactions are conditioned on meteorological catalysts, preventing spurious reaction predictions when conditions are unfavorable. The reactant interaction is captured via Self-Attention, while the sigmoid gate acts as a reaction rate coefficient $k$, activating the reaction only under favorable meteorological conditions (e.g., high UV radiation). 

The final drift function is the sum of these components: $\mathcal{F}_{drift} = \delta_{diff} + \delta_{adv} + \mathcal{R}_{chem}$.

\subsection{Neural Kalman Fusion}
To optimally integrate the physics-based prior and the data-driven measurement, we employ a Neural Kalman Filter \cite{DBLP:journals/tsp/RevachSNESE22} at each timestep. To ensure computational tractability for high-dimensional sensor networks, we adopt a Diagonalized Ensemble approach, assuming spatial independence in the instantaneous error covariance update. This reduces the complexity from $O(N^3)$ to $O(N)$.

\textbf{1. Prediction (Time Update):} The UDE solver integrates Eq. \ref{eq:ude_master} starting from the previous posterior $\mathbf{S}^+_{t-1}$ to generate the prior mean $\mathbf{S}^-_t$. Simultaneously, a variance estimator network predicts the process uncertainty $\mathbf{P}^-_t = \text{Softplus}(\text{MLP}(\mathbf{S}^-_t))$.

\textbf{2. Correction (Measurement Update):} We compute the optimal Kalman Gain $\mathbf{K}_t$ and update the state:
\begin{align}
    \mathbf{K}_t &= \frac{\mathbf{P}^-_t}{\mathbf{P}^-_t + \mathbf{R}_{obs, t}} \\
    \epsilon_t &= \mathbf{Z}_{obs, t} - \mathbf{S}^-_t \quad (\text{Innovation}) \\
    \epsilon'_t &= \epsilon_t + \text{MLP}_{corr}([\mathbf{S}^-_t, \mathbf{Z}_{obs, t}]) \quad \\ 
    \boldsymbol{\epsilon}'_t = \boldsymbol{\epsilon}_t + \text{MLP}_{corr}([\boldsymbol{\epsilon}_t, \mathbf{S}^-_t, \mathbf{R}_{obs, t}])
    (\text{Neural Correction}) \\
    \mathbf{S}^+_t &= \mathbf{S}^-_t + \mathbf{K}_t \odot \epsilon'_t \label{eq:posterior}
\end{align}
The introduction of the neural correction term $\epsilon'_t$ extends the standard Kalman filter to handle non-Gaussian residuals typical in complex atmospheric systems.

\textbf{3. Feedback Loop:} Crucially, the posterior state $\mathbf{S}^+_t$ serves as the initial condition for the UDE in the subsequent step ($t \to t+1$). This \textit{closed-loop mechanism} continuously corrects the physics trajectory using data-driven insights, effectively mitigating the error accumulation problem inherent in long-term open-loop forecasting.

\textbf{4. Handling Open System Dynamics:} A critical challenge in regional air quality modeling is the "Open System" problem, where pollutants diffuse out of the graph boundaries, violating mass conservation in standard closed-system physics models. Instead of adding explicit boundary terms, we model boundary leakage and unobserved sources as non-Gaussian process noise. The \textbf{Neural Correction} term $\epsilon'_t$ in Eq. \ref{eq:posterior} is explicitly designed to learn these residuals, dynamically compensating for the physical model's inability to track mass crossing the sensor network boundaries.

Finally, a decoder maps the sequence of posterior states to the target pollutant concentration: $\hat{\mathbf{Y}} = \text{Decoder}(\mathbf{S}^+_{1:T_{out}})$.

\subsection{Objective Function}
The entire framework is trained end-to-end by minimizing a composite loss function:
\begin{equation}
    \mathcal{L}_{total} = \mathcal{L}_{mae}(\hat{\mathbf{Y}}, \mathbf{Y}) + \lambda_{unc}\mathcal{L}_{nll}(\mathbf{S}^+, \mathbf{P}^+, \mathbf{Y}) + \lambda_{phy}||\mathcal{F}_{drift}||_2
    \label{eq:total_loss}
\end{equation}
where $\mathcal{L}_{nll}$ is the Negative Log-Likelihood loss to enforce probabilistic reliability, and the regularization term ensures the physical plausibility of the learned drift dynamics. We additionally use MAE as a 'guiding loss' to help the model converge faster to the mean in the early stages, since NLL is sensitive to noise.

\subsection{Training Paradigm}
To address exposure bias and "cold start" instability, we utilize Scheduled Sampling. During early training, the input state to the Process Model is sampled from the data-driven proxy $\text{StopGrad}(\mathbf{Z}_{obs})$ (acting as pseudo-ground truth) instead of the noisy posterior $\mathbf{S}^+$, with a probability that decays exponentially over epochs. This stabilizes the initial trajectory learning before transitioning to full closed-loop autonomy.
In Diffusion - Advection functions, we enforce physical laws and solver stability by constraining diffusion and advection coefficients to be non-negative via \texttt{Softplus} activation.

==> sections/preliminaries.tex <==
% \section{Preliminaries}
% \label{sec:preliminaries}

% In this section, we define the fundamental concepts and formulate the problem of secondary pollutant forecasting as a stochastic, physics-informed dynamical system.

% \begin{definition}
%     \textbf{Spatio-temporal Sensor Network.}
%     A spatio-temporal sensor network is represented as a static graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V} = \{v_1, \dots, v_N\}$ is a set of $N$ nodes (i.e., monitoring stations), and $\mathcal{E}$ is a set of edges representing the spatial relationships between the stations
% \end{definition}

% \begin{definition}
%     \textbf{Multivariate Observational State.}
%     The observational state of the network at a time step $t$ is a matrix $\mathbf{X}_{t} \in \mathbb{R}^{N \times D}$. Each row, corresponding to a node $v_i \in \mathcal{V}$, is described by a $D$-dimensional feature vector, which comprises:
%     \begin{itemize}
%         \item $\vec{C}_t^{(i)} \in \mathbb{R}^{D_C}$: A vector of pollutant concentrations (e.g., $PM_{2.5}, O_3, NO_x$).
%         \item $\vec{M}_t^{(i)} \in \mathbb{R}^{D_M}$: A vector of meteorological variables (e.g., temperature, wind).
%         \item $\vec{E}_t^{(i)} \in \mathbb{R}^{D_E}$: A vector of precursor emissions data (e.g., $VOCs, SO_2, NH_3$).
%     \end{itemize}
%     A historical sequence of states over $T_{in}$ time steps is denoted as $\mathbf{X}_{1:T_{in}} \in \mathbb{R}^{T_{in} \times N \times D}$.
% \end{definition}

% \begin{definition}
%     \textbf{Augmented System State.}
%     To explicitly model the delayed formation of secondary pollutants, we define an augmented system state $\mathbf{S}_t \in \mathbb{R}^{N \times (D_C + D_m)}$. This state includes the target pollutant concentrations $\mathbf{C}_t \in \mathbb{R}^{N \times D_C}$ and a set of $D_m$ chemical memory states $\mathbf{M}^m_t \in \mathbb{R}^{N \times D_m}$, which approximate the delayed impact of precursors.
%     \begin{equation}
%         \mathbf{S}_t = [\mathbf{C}_t, \mathbf{M}^m_t]
%     \end{equation}
% \end{definition}

% \begin{definition}
%     \textbf{Governing Physical Dynamics (SD-RAD System).}
%     We model the evolution of the augmented state $\mathbf{S}_t$ via a Stochastic Delay Reaction-Advection-Diffusion (SD-RAD) system on the graph $\mathcal{G}$. This system is represented by a Stochastic Differential Equation (SDE):
%     \begin{equation}
%         d\mathbf{S}_t = f(\mathbf{S}_t, \mathbf{X}_t, \Theta_{phy}) dt + g(\mathbf{S}_t, \mathbf{X}_t, \Theta_{noise}) dW_t
%         \label{eq:sde_system}
%     \end{equation}
%     where:
%     \begin{itemize}
%         \item $f(\cdot)$ is the deterministic drift function, parameterizing the physical processes (diffusion, advection, non-linear reaction, emissions, and memory dynamics).
%         \item $g(\cdot)$ is the stochastic diffusion function, modeling system noise and uncertainty (e.g., from wind or emission variability).
%         \item $dW_t$ is a standard Wiener process (Ito noise).
%         \item $\Theta_{phy}$ and $\Theta_{noise}$ are the learnable parameters of the physical system (e.g., reaction rates $k$, diffusion coefficients $D$, delay rates $\gamma$, and noise covariance $\sigma$) that are inferred from data.
%     \end{itemize}
% \end{definition}

% To construct the drift function $f(\cdot)$ for the discrete sensor network $\mathcal{G}$, we define discrete analogues for the spatial differential operators.

% \begin{definition}
%     \textbf{Graph Differential Operators.}
%     Given a node-defined function $\mathbf{f} \in \mathbb{R}^{N}$ (e.g., concentration):
%     \begin{itemize}
%         \item \textbf{Graph Gradient ($\nabla_{\mathcal{G}}$):} Computes the difference across edges.
%             \begin{equation}
%                 (\nabla_{\mathcal{G}} \mathbf{f})_e = f_j - f_i, \quad \text{for an edge } e=(i,j)
%                 \label{eq:graph_gradient}
%             \end{equation}
           
%         \item \textbf{Graph Divergence ($\nabla_{\mathcal{G}}\cdot$):} Computes the net flow at each node from an edge-defined vector field $\mathbf{v} \in \mathbb{R}^{|\mathcal{E}|}$ (e.g., pollutant flux).
%             \begin{equation}
%                 (\nabla_{\mathcal{G}}\cdot \mathbf{v})_i = \sum_{e \text{ incident to } i} v_e
%                 \label{eq:graph_divergence}
%             \end{equation}
           
%     \end{itemize}
%     The graph Laplacian operator, $\mathbf{L}_{\mathcal{G}} = \nabla_{\mathcal{G}}\cdot \nabla_{\mathcal{G}}$, is derived from these and is essential for the diffusion term.
% \end{definition}

% \begin{definition}
%     \textbf{Spatio-temporal Probabilistic Forecasting Function.}
%     A spatio-temporal probabilistic forecasting function, $f_{\Theta}$, is a mapping parameterized by $\Theta$ that takes the historical state sequence $\mathbf{X}_{1:T_{in}}$ and the graph $\mathcal{G}$ as input, and outputs a future forecast probability distribution $p(\mathbf{\hat{Y}})$ for the concentrations $\mathbf{\hat{Y}}_{T_{in}+1:T_{in}+T_{out}} \in \mathbb{R}^{T_{out} \times N \times D_C}$ over the next $T_{out}$ time steps.
%     \begin{equation}
%         f_{\Theta}: (\mathbf{X}_{1:T_{in}}, \mathcal{G}) \mapsto p(\mathbf{\hat{Y}}_{T_{in}+1:T_{in}+T_{out}})
%         \label{eq:prob_forecasting_function}
%     \end{equation}
%     In our framework, $f_{\Theta}$ learns to infer the SDE parameters $(\hat{\Theta}_{phy}, \hat{\Theta}_{noise})$ and integrates Eq. \ref{eq:sde_system} to produce this distribution (e.g., $\mathcal{N}(\mu_{phy}, \Sigma_{phy})$).
% \end{definition}

% \begin{definition}
%     \textbf{Physical Constraint Residuals.}
%     To ensure the forecasts from $f_{\Theta}$ are physically sound and reliable, we define a set of constraint residuals:
%     \begin{itemize}
%         \item \textbf{Dynamics Residual ($\mathcal{R}_{\mathcal{P}}$):} Measures the violation of the deterministic drift $f(\cdot)$ of the governing SDE.
%             \begin{equation}
%                 \mathcal{R}_{\mathcal{P}}(\mathbf{\hat{Y}}, \hat{\Theta}_{phy}) = \left\| \frac{\partial \mathbf{\hat{Y}}}{\partial t} - f(\mathbf{\hat{Y}}, \mathbf{X}, \hat{\Theta}_{phy}) \right\|
%             \end{equation}
%         \item \textbf{Mass Balance Residual ($\mathcal{R}_{Mass}$):} Evaluates the system-wide conservation of mass, comparing the total change in pollutant mass against emissions and deposition sinks.
%         \item \textbf{Uncertainty Calibration Residual ($\mathcal{R}_{Unc}$):} Measures the quality of the forecast distribution $p(\mathbf{\hat{Y}})$, e.g., via the Continuous Ranked Probability Score (CRPS) or Negative Log-Likelihood (NLL).
%     \end{itemize}
%     A forecast is considered physically consistent and reliable when all residuals approach zero.
% \end{definition}

% \vspace{0.5cm}

% \textbf{Problem Definition.} \textit{Given a spatio-temporal sensor network $\mathcal{G}$ and a historical multivariate state sequence $\mathbf{X}_{1:T_{in}}$, our objective is to learn a probabilistic forecasting function $f_{\Theta}$ (Eq. \ref{eq:prob_forecasting_function}). The function $f_{\Theta}$ must be optimized to simultaneously satisfy four criteria:
% \begin{enumerate}
%     \item \textbf{Accuracy:} Minimize the empirical prediction error (e.g., MAE) against ground-truth observations $\mathbf{Y}$.
%     \item \textbf{Reliability:} Minimize the uncertainty calibration residual $\mathcal{R}_{Unc}$ to ensure the forecast distribution is reliable.
%     \item \textbf{Dynamics Consistency:} Minimize the dynamics residual $\mathcal{R}_{\mathcal{P}}$ by inferring physically plausible parameters $\hat{\Theta}_{phy}$.
%     \item \textbf{Conservation Consistency:} Minimize the mass balance residual $\mathcal{R}_{Mass}$ to adhere to fundamental physical laws.
% \end{enumerate}}

% ###############################################################

\section{Preliminaries}
\label{sec:preliminaries}

% In this section, we establish the mathematical notations and formulate the air quality forecasting task as a problem of optimal state estimation within a Universal Stochastic Dynamical System.

\begin{definition}
    \textbf{Spatio-temporal Sensor Network.}
    The monitoring network is represented as a weighted static graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathbf{A})$, where $\mathcal{V} = \{v_1, \dots, v_N\}$ denotes the set of $N$ monitoring stations, and $\mathcal{E}$ represents the edges. $\mathbf{A} \in \mathbb{R}^{N \times N}$ is the weighted adjacency matrix encoding spatial correlations (e.g., geographical proximity) between stations.
\end{definition}

\begin{definition}
    \textbf{Edge Direction Vector.} For every connected pair of nodes $(v_i, v_j) \in \mathcal{E}$, we define the unit direction vector $\vec{e}_{ij} \in \mathbb{R}^2$ representing the geometric orientation of the transport pathway from source $i$ to target $j$:
\begin{equation}
    \vec{e}_{ij} = \frac{\text{pos}_j - \text{pos}_i}{||\text{pos}_j - \text{pos}_i||_2}
\end{equation}
where $\text{pos}_i, \text{pos}_j$ denote the spatial coordinates of the monitoring stations. This vector is critical for projecting the wind velocity field onto the graph topology in the anisotropic advection module.
\end{definition}

\begin{definition}
    \textbf{Multivariate Observational Time series.}
    At each time step $t$, the system's observational state is denoted as $\mathbf{X}_{t} \in \mathbb{R}^{N \times D_{in}}$. Each node $v_i$ is associated with a feature vector comprising three distinct components:
    \begin{itemize}
        \item \textbf{Pollutant Concentrations ($\mathbf{C}_t$):} The target variables (e.g., $PM_{2.5}$) and related co-pollutants (e.g., $O_3, NO_x$).
        \item \textbf{Meteorological Conditions ($\mathbf{M}_t$):} Environmental drivers including scalar fields (e.g., temperature, humidity, solar radiation) and vector fields (e.g., wind speed and direction).
        \item \textbf{Emission Rates ($\mathbf{E}_t$):} The flux of precursor emissions (e.g., $NO_x$, $VOCs$, and $SO_2$) from anthropogenic sources.
    \end{itemize}
    We denote the historical sequence over an input window $T_{in}$ as $\mathbf{X}_{1:T_{in}} \in \mathbb{R}^{T_{in} \times N \times D_{in}}$.
\end{definition}

% \begin{definition}
%     \textbf{Latent State Space.}
%     To model unobserved dynamics (e.g., intermediate chemical species) and reduce computational complexity, we project the high-dimensional observations into a lower-dimensional latent state space. The latent state at time $t$ is denoted as $\mathbf{S}_t \in \mathbb{R}^{N \times D_{state}}$, which serves as the evolving variable in the differential equations and Kalman filtering process.
% \end{definition}
% \begin{definition}
%     \textbf{Traditional physical SDEs} 
    
    
\end{definition}
% \begin{definition}
%     \textbf{Universal Process Model.}
%     The temporal evolution of the latent state $\mathbf{S}_t$ is governed by a Universal Stochastic Differential Equation (UDE). Unlike traditional physical SDEs, the UDE integrates deep neural networks to approximate unknown dynamics:
%     \begin{equation}
%         d\mathbf{S}_t = \underbrace{f_{\theta}(\mathbf{S}_t, \mathbf{U}_t, \mathcal{G})}_{\text{Drift Function}} dt + \underbrace{g_{\phi}(\mathbf{S}_t)}_{\text{Diffusion Function}} d\mathbf{W}_t
%         \label{eq:universal_sde}
%     \end{equation}
%     where:
%     \begin{itemize}
%         \item $\mathbf{U}_t = [\mathbf{E}_t, \mathbf{M}_t]$ represents the time-varying external forcing terms (emissions and meteorology) that drive the system.
%         \item $f_{\theta}(\cdot)$ is the learnable drift function, explicitly decomposing the dynamics into known physical transport (advection-diffusion) and unknown chemical kinetics (approximated by neural networks).
%         \item $g_{\phi}(\cdot)$ models the state-dependent process noise, and $\mathbf{W}_t$ is a standard Wiener process.
%     \end{itemize}
% \end{definition}

% To explicitly model the physical transport component within $f_{\theta}$, we utilize graph differential operators:

% \begin{definition}
%     \textbf{Normalized Graph Laplacian.}
%     Given the adjacency matrix $\mathbf{A}$ and the degree matrix $\mathbf{D} = \text{diag}(\sum_j A_{ij})$, the normalized graph Laplacian is defined as $\mathbf{L} = \mathbf{I} - \mathbf{D}^{-1/2}\mathbf{A}\mathbf{D}^{-1/2}$. This operator is employed to model isotropic diffusion processes over the sensor network.
% \end{definition}

\textbf{Problem Formulation.}
\textit{Given the sensor graph $\mathcal{G}$ and the historical observation sequence $\mathbf{X}_{1:T_{in}}$, our objective is to learn a probabilistic forecasting function $F_{\Theta}$ that estimates the posterior distribution of future states:}
\begin{equation}
    p(\mathbf{X}_{T_{in}+1 : T_{in}+T_{out}} | \mathbf{X}_{1:T_{in}}, \mathcal{G})
    \label{eq:prob_forecasting_function}
\end{equation}






==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:related-work}

\noindent\textbf{Spatio-temporal Air Quality Forecasting.}
Early approaches in air quality forecasting primarily relied on statistical models like ARIMA \cite{DBLP:journals/kbs/Li0023} and VAR~\cite{DBLP:journals/tsp/ZamanLRB21}, which fail to capture non-linear spatiotemporal dependencies.
The advent of Deep Learning shifted the paradigm towards capturing complex patterns from data.
Recurrent Neural Networks (RNNs), such as LSTM and GRU, became standard for modeling temporal dependencies, while Convolutional Neural Networks (CNNs) were employed to extract spatial features from grid-based data.
To better model the non-Euclidean structure of sensor networks, Graph Neural Networks (GNNs) have emerged as a dominant approach.
Methods like DCRNN~\cite{DBLP:conf/iclr/LiYS018} and STGCN~\cite{DBLP:conf/ijcai/YuYZ18} integrate graph diffusion convolution with recurrent units to model spatiotemporal traffic dynamics, which were subsequently adapted for air quality in PM2.5-GNN~\cite{DBLP:conf/gis/WangLZMMG20} and GC-LSTM.
More recently, Transformer-based architectures, such as AirFormer~\cite{DBLP:conf/aaai/LiangXKWWZZZ23} and iTransformer \cite{DBLP:conf/iclr/LiuHZWWML24} , leverage self-attention mechanisms to capture long-range global dependencies.
Furthermore, State Space Models (SSMs), particularly Mamba~\cite{DBLP:journals/corr/abs-2312-00752}, have demonstrated superior efficiency in modeling extremely long sequences with linear complexity, outperforming Transformers in various benchmarks~\cite{DBLP:journals/corr/abs-2312-00752}.
However, these purely data-driven methods, despite their high accuracy in short-term horizons, operate as "black boxes" lacking physical constraints.
They often suffer from error accumulation (drift) in long-term forecasting and fail to generalize to out-of-distribution scenarios, such as sudden secondary pollution events driven by unobserved chemical kinetics.

\noindent\textbf{Physics-Informed Machine Learning (PIML).}
PIML aims to integrate fundamental physical laws into deep learning models to enhance interpretability and generalizability.
A foundational approach is Physics-Informed Neural Networks (PINNs)~\cite{DBLP:journals/jcphy/RaissiPK19}, which embed Partial Differential Equations (PDEs) into the loss function as soft constraints.
However, optimizing PINNs for complex, chaotic atmospheric dynamics is notoriously difficult due to the landscape of the regularization loss.
An alternative paradigm, Neural Ordinary Differential Equations (Neural ODEs)~\cite{DBLP:conf/nips/ChenRBD18}, parameterizes the derivative of the hidden state with neural networks, naturally modeling continuous-time dynamics.
Recent works have successfully applied this to atmospheric sciences.
AirPhyNet~\cite{DBLP:conf/iclr/HettigeJXLCW24} models diffusion and advection using graph-based ODEs but assumes a closed system, neglecting boundary fluxes.
Air-DualODE~\cite{DBLP:conf/iclr/TianL0CGZPRY25} addresses this by introducing a dual-branch architecture for open systems, employing a dynamic advection graph and a contrastive alignment strategy.
Simultaneously, Universal Differential Equations (UDEs)~\cite{DBLP:journals/corr/abs-2001-04385} have generalized this concept by allowing neural networks to approximate missing terms in physical equations.
Despite these advancements, existing PIML models for air quality often oversimplify the \textit{reaction} term (e.g., using linear coefficients or independent MLPs) and treat the physics and data branches as parallel processes fused only at the output level.
This "loose coupling" prevents the data branch from continuously correcting the physics trajectory, limiting robustness in long-horizon forecasting.

\noindent\textbf{Deep Data Assimilation and Kalman Filtering.}
Data Assimilation (DA) is the gold standard in numerical weather prediction for combining noisy observations with imperfect physical models.
Traditional methods like the Ensemble Kalman Filter (EnKF) are computationally expensive and rely on explicit, often unknown, error covariance matrices.
Deep learning has recently reinvigorated this field by learning these components from data.
KalmanNet~\cite{DBLP:journals/tsp/RevachSNESE22} proposes a hybrid architecture where the Kalman Gain is computed dynamically by a neural network, allowing for optimal fusion in partially known dynamics.
Similarly, differentiable particle filters have been explored for non-linear state estimation.
However, the application of Deep Kalman Filtering in spatiotemporal air quality forecasting remains underexplored.
Most existing works use Kalman filters merely for post-processing or simple bias correction.
In contrast, our work, \framework, is the first to integrate a Universal Differential Equation (modeling complex transport and chemical kinetics) with a Neural Kalman Filter in a \textit{closed-loop autoregressive} manner.
This design allows the model to leverage the global context from S-Mamba to continuously rectify the physical state, effectively mitigating long-term drift and improving secondary pollutant prediction.
